Prompt-SAW: Leveraging Relation-Aware Graphs for Textual Prompt Compression

Large Language Models (LLMs) have shown exceptional abilities for multiple different natural language processing tasks. While prompting is a crucial tool for LLM inference, we observe that there is a significant cost associated with exceedingly lengthy prompts. Existing attempts to compress lengthy prompts lead to substandard results in terms of readability/interpretability of the compressed prompt, with a detrimental impact on prompt utility. To address this, we propose PromptSAW: Prompt compresSion via Relation AWare graphs, an effective strategy for prompt compression over task-agnostic and task-aware prompts. Prompt-SAW uses the prompt's textual information to build a graph and later extracts key information elements in the graph to come up with the compressed prompt. We also propose GSM8K-aug, i.e., an extended version of the existing GSM8K benchmark for task-agnostic prompts in order to provide a comprehensive evaluation platform. Experimental evaluation using benchmark datasets shows that prompts compressed by Prompt-SAW are not only better in terms of readability, but they also outperform the best-performing baseline models by up to 10.1 and 77.1, respectively, for task-agnostic and task-aware settings while compressing the original prompt text by 34.9 and 56.7.

==> Figure_tex/fig3.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{Figure/GSM8K-1-shot.pdf}
    \vspace{-2.7ex}
    \caption{EM changes with compression ratio on GSM8K.}
    \vspace{-2.7ex}
    \label{fig:ratio}
\end{figure}

==> Table_tex/alg1.tex <==

\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
    \caption{\scshape Subgraph Extraction }
    \label{alg:alg1}
    \begin{algorithmic}[1]
    \Require
        \item[] { \#$\eta^{*}:$ {Target compression rate}}
        \item[] { \#$\mathcal{G}:$ Graph structure of prompt}
        \item[] { \#$len():$ Compute the length of graph structure, as the sum of individual tokens.}
    \Ensure subgraph $\mathcal{G}_{subset}$
        \State $\mathcal{G}_{subset}=\{\}$
        \For{$i \in Index_{\text{ranked}}$}
        \State $\mathcal{G}_{subset}.insert(g_i)$
        \State { \#compute compression rate}
        \State $Rate= len(\mathcal{G}_{subset})/len(\mathcal{G})$
        \State { \#break if meet the constraint}
        \State $\mathbf{If}$ $Rate> \eta^*$ \textbf{then}
        \State $ \qquad Break$
        \State \textbf{end If}
        \EndFor
        \State \Return $\mathcal{G}_{subset}$
    \end{algorithmic}
\end{algorithm}
\end{minipage}
   \hfill
\begin{minipage}{0.46\textwidth}
\begin{algorithm}[H]
    \caption{\scshape Binary Search}
    \label{alg:alg2}
    \begin{algorithmic}[1]
    \Require
        \item[] { \#$\eta^{*}:$ {Target compression rate}}
        \item[] { \#$\mathcal{G}:$ Graph structure of prompt}
        \item[] { \#$\gamma:$ interval threshold}
    \Ensure subgraph $\mathcal{G}_{subset}$
        \State double $l=0,r=1$
        \While{$r-l > \gamma$}
        \State double $mid=(l+r)/2$
        \State $\mathcal{G}_{subset} = Compress(\mathcal{G},mid)$
        \State $Rate= len(\mathcal{G}_{subset})/len(\mathcal{G})$
        \State $\mathbf{If}$ $Rate > \eta^{*}$ \textbf{then}
        \State $ \qquad r=mid$
        \State \textbf{Else} 
        \State $ \qquad l=mid$
        \EndWhile
        \State $\delta=(l+r)/2$  \# compression threshold
        \State $\mathcal{G}_{subset} = Compress(\mathcal{G},\delta)$
        \State \Return $\mathcal{G}_{subset}$
    \end{algorithmic}
\end{algorithm}
\end{minipage}


==> Table_tex/exp3.tex <==
\begin{table}[h]
% \begin{tabular}{@{}lllllcccccc@{}}
\centering
\renewcommand{\arraystretch}{1.5}
\resizebox{0.90\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Target   LLMs} & \multicolumn{3}{c}{GSM8K-AUG} & \multirow{2}{*}{Natural Questions} \\ \cmidrule{2-4}
                            & 1shot    & 2shot   & 4shot & \\ 
\midrule
GPT3.5                      & 67.83    & 72.00   & 72.12  & 73.22                             \\
GPT4                        & 91.48    & 93.17   & 95.92  & 74.36                             \\ 
\bottomrule
\end{tabular}
}
% \end{table}
\caption{The performance comparison  of~\OurMODEL{} 
using different target LLMs. \di{What is $\eta^*$?}} 
\label{tab:exp3}
\vspace{-2.1ex}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/XX4_Benchmark.tex <==
\section{Benchmark:xxx}
We construct the benchmark benchmarkname. Our benchmark is meticulously crafted to concentrate on prompt compression in the few-shot chain-of-thought (CoT) scenarios, given their prevalence as the primary contributors to excessively lengthy prompts. Initially, we outline the data construction process for benchmarkname, providing an overview of the data statistics and evaluation settings thereafter. Finally, we elaborate on the evaluation metrics utilized.

\subsection{Data Construction of bencmarkname}
Our benchmark comprises two components: \textbf{Prompts} and \textbf{Questions}. Each prompt is methodically paired with every question throughout the evaluation process to create an extensive array of tests, culminating in the final results. The prompts are carefully designed by humans, and the questions are constructed based on GSM8K and BBH datasets.
\subsubsection{Dataset Introduction}
\textbf{GSM8K}(\cite{GSM8K}) GSM8K is a widely utilized dataset for evaluating mathematical reasoning, consisting of 8,500 high-quality, human-constructed problems in elementary mathematics. Its primary purpose is to assess the inferential capabilities of generative language models.

\textbf{BIG-Bench Hard}(\cite{BBH}) BIG-Bench Hard is a suite of language and symbolic reasoning tasks, which consisting 6.5k problems and focuses on 23 challenging tasks. The tasks encompassed by the BIG-Bench Hard framework necessitate multi-step reasoning for successful completion, rendering it exceptionally well-suited for evaluating the efficacy of chain-of-thought prompting.

  
\subsubsection{Data Construction of Prompt}
Drawing on previous research(\cite{ChainofThoughtHub}), we meticulously designed prompts of varying difficulty levels for a thorough evaluation. The complexity of a prompt is gauged by two criteria: the step in the chain-of-thought (CoT) and the number of shots within the prompt. Each prompt was carefully crafted by hand.

\subsubsection{Data Construction of Question}
Upon completing the construction of prompts, we identified the most challenging and the simplest prompts for question construction, designated as $P_{hard}$ and $P_{easy}$, respectively. We applied various prompt compression algorithms, generating two distinct sets of prompts: $S_{hard}=\{P_{hard}\}\cup\{p_{hard}^i\mid i\in\mathbb{N},1\leq i\leq N\}$, where $P_{hard}$ signifies the original prompt and $P_{hard}^i$ represents the variants created through the application of prompt compression algorithms. $N$ represents the number of compression algorithms employed. A similar approach was employed to construct $S_{easy}$ based on $P_{easy}$.

We tested all questions using all prompts in the $S_{hard}$ and removed those questions that were incorrectly answered across all prompts, as we believe these questions are inherently too difficult, and incorrect answers do not necessarily indicate poor compression performance.

Following the same procedure, assessments were conducted on the $S_{easy}$, and questions that were correctly answered in all prompts were removed. This is because we believe these questions are inherently too simple, and correctly answering them does not necessarily indicate effective compression.

We conducted a manual screening of the remaining questions, eliminating duplicates to ensure broad coverage. 


\subsection{Dataset Summary}
% 
\textbf{Dataset format} As shown in Table I, each instance in the benchmark benchmarkname is denoted by tuple d=<P,Q>

\textbf{Data statistics}

\subsection{Evaluation Metrics}
Following \cite{LostInMiddle} and \cite{llmlingua}, we adopt accuracy as our principal evaluation metric, assessing the presence of correct answers within the predicted output.



==> section/XX_1_Introduction2.tex <==
\section{Introduction}
% background介绍
Large Language Models (LLMs) have attracted considerable attention for 
their superior performance across a wide range of applications. For 
this task-specific instructions (aka prompts) play a crucial role 
for extending the capabilities of LLMs for multiple different tasks.
The prompts provide the provision to guide the model to elucidate
desired model behavior without perturbing the model parameters.
This is also highlighted in recent studies that show well-designed 
prompts and the integration of external knowledge is significant 
to enhance the effectiveness of LLMs' (\citet{PromptEngineeringSurvey},~\citep{PromptEngineeringSurvey}).
Different LLMs-related techniques directly benefiting from prompts 
include but are not limited to: 
In-Context Learning (\citet{ICL},~\citep{ICL}), 
Chain-of-Thought (\citet{CoT},~\citep{CoT}), 
Retrieval Augmented Generation (\citet{RAG},~\citep{RAG}), 
and Agents (\citet{Agent},~\citep{Agent}) etc. 
\eat{play a crucial role in this process.}







% 引出prompt压缩
%(\citet{softPrompt}~\citep{softPrompt})
At the same time, the abilities of LLMs are significantly 
compromised/constrained by increasingly lengthy prompts, 
even comprising thousands of tokens. 
Lengthy prompts 
not only obscure requisite/essential information, but
also increase the computational costs and incur inference latency.
To tackle this challenge, \textit{prompt compression} 
techniques, e.g.,~\cite{selectiveContext}, have garnered significant interests.
These approaches are based on the fact that natural language is 
inherently redundant~(\citet{rongyu}~\citep{rongyu}) and we may 
substantially compress the length of original textual prompts by preserving 
requisite/essential information (\citet{softPrompt},~\citep{softPrompt})
in way that it maintains and/or improves the end-utility of the prompt.

\eat{These approaches are \eat{predicated}\asif{based} on the \eat{notion}\asif{fact} 
that natural language inherently contains redundancies~\cite{rongyu}, 
seeks to diminish the length of the original prompts.
~\cite{softPrompt} observed that such compressed 
prompts are capable of preserving essential information.}

% 介绍已有方法
Existing prompt compression approaches may be divided into 
two major categories: soft prompt compression
~(\citet{softPrompt},~\citep{softPrompt}) and 
discrete prompt compression~(\citet{Jung2023DiscretePC},~\citep{Jung2023DiscretePC}).
Soft prompt compression employs back-propagation to incorporate information from 
labeled training instances. It suffers from lack of cross-model reusability 
and is ineffective for proprietary LLMs (only accessible via APIs). 
On the other hand, discrete prompt compression exploits the discrete nature 
of the text to design strategies that directly changes/edits the prompt tokens.
For instance,~\cite{selectiveContext} proposed Selective-Context that uses 
a compact language model to evaluate context's lexical units, enabling 
compression by eliminating units with minimal information. 
Also, LLMLingua~(\citet{llmlingua},~\citep{llmlingua}) 
and LongLLMLingua~(\citet{longllmlingua},~\citep{longllmlingua}) 
developed budget control mechanisms to compresses prompts based on their perplexity.


\fixme{some limitations of discrete prompting methods..? \warn{Add in red plz.}}

\eat{Prompt compression technologies are currently divided into two main categories: soft prompt compression~\cite{softPrompt} and discrete prompt compression~\cite{Jung2023DiscretePC}. Soft prompt compression, achieved by training embeddings inclusive of the original context, suffers from a lack of cross-model reusability and is ineffective when Large Language Models (LLMs) are accessible only via APIs. Conversely, a more promising strategy involves directly compressing discrete prompts that consist of specific tokens from the vocabulary.
~\cite{selectiveContext} propose Selective-Context, employs a compact language model to evaluate the self-information of context's lexical units, enabling compression through the elimination of units with minimal informational value. Subsequently, LLMLingua~\cite{llmlingua} and LongLLMLingua~\cite{longllmlingua} developed an innovative budget control mechanism and compresses prompts based on their perplexity.} 

% 引出limitation
\warn{We observe the existing research on prompt compression \eat{encounters}
lacks two key/primary aspects, i.e., evaluation fairness and grammatical structural coherence.}

\eat{These methodologies encounter two primary challenges: evaluation fairness and 
\eat{structural deficiency}~\asif{grammatical structural coherence}.}
% Prompt压缩算法对不同的Prompt压缩结果有较大的方差，但是目前Prompt压缩算法选择的基准Prompt数量较少，这会导致结果的偏移。而且他们没有基于相同的基准Prompt进行压缩，这也进一步加剧了不公平性。
\warn{The evaluation fairness implies absence of a universally accepted benchmark 
for rigorous \eat{prompt compression results in} evaluation 
\eat{not being conducted}under equitable conditions.}
\eat{\asif{Lacking evaluation fairness implies absence of a universally accepted benchmark 
for rigorous \eat{prompt compression results in} evaluation 
\eat{not being conducted}under equitable conditions.}}
\warn{The performance of compression algorithms\eat{for prompts} varies significantly in terms of the outcomes of compressed prompts.
However, the range of original prompts selected by these algorithms is restricted, 
resulting in biased outcomes. \fixme{Double-check. What do you mean here..?}
Furthermore, the absence of standardized benchmark prompts across algorithms 
amplifies the issue of unfair comparisons.}

\textbf{Do we also work out transfer-ability of compressed prompts
across different LLMs..??}
\fixchen{Do we really solve this...? Do we set up a standard benchmark 
+ Evaluate all existing approaches. If not we need to mention other limitations.}

% 这不仅使得压缩后的Prompt存在语义缺失的风险，而且会造成压缩后的Prompt人类进行阅读存在困难。
\warn{By structural coherence, we imply existing approaches neglect the 
syntactic and semantic structure of the compressed prompt thus hampering 
its readability for the human readers. 
It happens because the contemporary prompt compression algorithms primarily 
focus on quantifying token-level information, neglecting the overall 
grammatical structure of the compressed prompt.}
\fixchen{It would be best if we could add an output example in introduction, 
showing lack of grammatical structures for output of any existing PC techniques}

\eat{Secondly, contemporary prompt compression algorithms primarily focus on 
quantifying token-level information content, neglecting the overall structural 
information of the prompt. This not only increases the risk of semantic loss 
within the compressed prompt but also hampers its readability for human readers.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Apart from this, we observe compressing longer prompts into short 
concise and meaningful 
text is a challenging task. An effective prompt compression strategy 
has to preserve the requisite semantic content while at the same time 
maintaining the end-performance.
It is very hard to enforce stringent constraints on the
compressed prompt, as overly-concise prompts may 
result in losing requisite semantic contents, eventually 
leading to performance degradation.
Moreover, the discrete nature of the text makes it difficult to use 
back-propagation for effective gradient propagation.


% 介绍自己的方法
To address these challenges, in this paper we propose 
\textsc{\underline{\textbf{Prompt}}} 
compres\underline{\textbf{S}}ion 
using relation \underline{\textbf{AW}}are graphs (\OurMODEL{}), 
a novel method designed to cut-down un-necessary information in the 
prompt text by exploiting knowledge graph relational triplets.
\warn{Specifically,~\OurMODEL{} first extracts all possible 
relational triplets for the information contained in the prompt.
Later, it organizes the relational triplets as meaningful and 
semantically coherent sentence structures helpful for identifying 
superfluous information. Finally, it, reinstates essential knowledge 
graph triples, resulting in an optimized and compressed prompt.
}


%%%%%%%%%%%%%%%%%%


\asif{\OurMODEL{} attained state-of-the-art performance on open-source evaluation 
benchmarks, i.e.,~\textsc{GSM8K} and \textsc{BBH}. Note, the existing benchmarks 
are limited to a small range of tasks~\warn{(also explained in Section XX)}, 
we also curated a novel benchmark namely \fixchen{NAME of Benchmark} 
encompassing prompts from diverse task scenarios for a rigorous 
evaluation of \OurMODEL. We summarize the key contributions of this work as follows:}

\warn{
\begin{itemize}
    \item We propose~\OurMODEL{}, a methodology crafted for compressing prompts 
    by extracting the graph-structured information embedded within the prompts themselves.
    \item We establish a benchmark for the evaluation of prompt compression.
    \item We carried out comprehensive experiments across a range of prompt compression algorithms, demonstrating that our approach achieves state-of-the-art performance.
\end{itemize}}
\fixme{Re-write the contribution based on the new proposed methodology.}
\li{Extended prompts result in elevated costs and inference delays. Moreover, they can contribute to a potential decline in model performance}







%%%%%%%%%%%%%%%% EXTRA Text %%%%%%%%%%%%%%%%%%%%%%%%



\eat{\OurMODEL{} attained state-of-the-art performance on open-source data sets, i.e.,  
\textsc{GSM8K} and \textsc{BBH}. 
Given the fact
During the experimentation phase, it became clear that a single dataset provided a limited range of tasks and lacked a suitable original prompt for fair comparison. 
We also developed
Consequently, we developed a benchmark comprising initial prompts alongside diverse task scenarios.}



\eat{To address these challenges, in this paper we propose \textbf{K}nowledge 
\textbf{G}raph \textbf{B}ased \textbf{P}rompt \textbf{C}ompression (\OurMODEL), 
a novel method designed for prompt compression through the extraction 
of graph structure information.
\eat{, aiming to resolve the aforementioned issues}
Specifically,~\OurMODEL{} first extracts all possible 
\eat{knowledge graph triples or} relational triplets for 
the information contained in the prompt.
\eat{to eliminate redundant semantic information within the prompt.}
Later, it \eat{\textsc{KGBPC} further} organizes the relational
triplets as meaningful and semantically coherent sentence structures 
helpful for identifying\eat{and removing} superfluous information.
\eat{enhances prompt conciseness by relational triples leveraging graph structure insights.}
In the concluding phase, \textsc{KGBPC} reinstates essential knowledge graph triples, resulting in an optimized and compressed prompt.
}


\eat{Despite their advantages, LLMs sometimes face issues like logical errors and factual inaccuracies, which limits their real-world applicability (\citet{Hallucination},~\citep{Hallucination}).}


%\fixchen{Add some justifications for why we need compressed prompts? E.g., 
%(i) reduce inference latency, (ii) what else..!}

\eat{Nevertheless, these methods result in the use of increasingly lengthy prompts, 
even comprising thousands of tokens. Such lengthy prompts not only increase 
computational costs but also risk obscuring essential information, thereby 
diminishing the performance of LLMs.}


==> section/XX_5_Method2.tex <==
\section{KGBPC} 
\OurMODEL{} is a graph-based prompt compression method that can capture the overall semantic information of prompts using graph structures and determine the optimal compression ratio adaptively based on the information content. The core components of \OurMODEL{} include a graph structure information extractor and an adaptive compression ratio calculator. The workflow of \OurMODEL{} is summarized as follows: 1. Construct a graph from the original prompt. 2. Adaptively extract subgraphs from the graph based on the information content. 3. Recover the natural language representation from the extracted subgraphs.

\subsection{Graph Construction}
The ultimate goal of the graph construction process is to propose a mechanism to represent the information of the original prompt in a more structured manner. We posit that this extraction process facilitates the initial removal of redundant information from the original prompt. 

The graph construction process takes the original prompt  $\mathcal{P}_t$ as input and generates a graph $\mathcal{G}_{t}$ as output. The representation of structured information in the form of $\textless{}s, r, o\textgreater{}$ is highly effective. Therefore, the initial step involves decomposing the prompt into multiple instances of $\textless{}s, r, o\textgreater{}$ format.

This step constructs the $\textless{}s, r, o\textgreater{}$ tuple, which itself filters out redundant information. However, semantic duplication still persists across different $\textless{}s, r, o\textgreater{}$ tuples. Consequently, it is necessary to further fuse them. Fusion involves employing any metric related to distance. In this work, the technique utilized merges nodes sharing identical values of $s$ and $r$.
We embed all the fused $\textless{}s, r, o\textgreater{}$, and use the embedded results as the vertices of the graph, thus obtaining $\mathcal{G}_{t}$.

\subsection{Adaptive subgraph extraction}
The prompt is specifically crafted to address the problem, necessitating the inclusion of relevant information in the initial diagram constructed during the first phase.

Due to the high information density of the problem itself, structuring the problem might result in the loss of some critical information. Therefore, we choose to set the problem as the super vertex of the graph directly. Specifically, we extract the problem $P_q$ in its entirety from the original prompt and then set the embedding result $E_q$ of $P_q$ as the super vertex 
$v_{super}$ of $\mathcal{G}_{t}$.


To perform subgraph extraction effectively, it is essential to evaluate the contribution of each vertex within $\mathcal{G}_{t}$ towards the super vertex and to isolate subgraphs that exhibit high contributions. This process involves establishing connections between all vertices in $\mathcal{G}_{t}$. The edge between $v_i$ and $v_j$ is denoted as $e_{ij}$, which can be represented as:
\begin{equation}
   e_{ij} = D(v_i, v_j)
\end{equation}
$D(\cdot)$ can be any metric related to similarity. In this work, we use cosine similarity as the metric.

Initially, we let the vertex set $S_{v}$ in final extracted subgraph as $\{v_{super}\}$, with its initial score designated as 0. Subsequently, we select the edge $e_k$ that has the highest value from those connected to the super-origin and incorporate its corresponding vertex $v_k$ into $S_v$. Following this, we compute the current score of the subgraph using the specified formula:
\begin{equation}
score_{k} = \frac{1}{k}\sum_{i=1}^k w(v_i,v_0)
\end{equation}
where $k$ denotes the extraction of the $k^{th}$ subgraph, while $v_i$ represents the $i^{th}$ element within $S_{v}.$
Next, we employ an adaptive compression rate calculator to ascertain whether to halt subgraph extraction and output or to persist in the extraction process.

We calculate the gap $\beta$ between the score of the current subgraph and the score of the subgraph from the previous round:
\begin{equation}
    \beta = \frac{score_k-score_{k-1}}{score_{k-1}}
\end{equation}
if $\beta > \eta$, persist in the extraction process; otherwise halt subgraph extraction,delete the final element in $S_v$ and output $S_v$. $\eta$ is a hyperparameter used to balance compression accuracy and compression ratio, a larger $\eta$ will lead to a higher compression ratio but may result in a potential decrease in compression accuracy, and vice versa.

\subsection{Recover from subgraph}
We employ mapping techniques to reconstruct the original natural language representation from $S_v$, denoted as $N_v$, subsequently deriving the final prompt through amalgamation. It is crucial to emphasize that while amalgamating, reliance on the scores outlined in Section 5.2 is unsuitable; instead, amalgamation should proceed according to the sequential order in which each vertex appears in the original prompt. Relying on scores for amalgamation may result in illogical transitions, thereby deteriorating prompt performance.

















































==> section/XX_5_Method3.tex <==
\section{Graph Based Prompt Compression} 
\subsection{The structure of natural language.}
\warn{What is structure?}\\
The structure of natural language refers to its systematic organizational form. (\citet{rongyu},\citep{rongyu}) \fixchen{Find some recent research!!!too old} posited that natural language is inherently redundant, thereby allowing for extracting substructures to eliminate redundant content.\\

\warn{What method we used to extract the structure? Why we need to mention syntactic and discourse structure?}\\

The structure of natural language can be specifically divided into syntactic structure and discourse structure. \\
\textbf{Syntactic structure.} Syntactic structure focuses on the combination of words within a single sentence. Extracting the core substructure of the syntactic structure can help us eliminate the redundancy inherent in natural language expression, such as grammatical modifications and synonymous repetition.\\
\textbf{Discourse structure.} Discourse structure concentrates on the organization of sentences and the distribution of information within a complete text. Removing redundancy from the discourse structure means identifying the most helpful substructures in answering the question.\\
\warn{What method we used to extract the structure?}


\eat{
\warn{Why the natural language sequence have graph structure?}\\
\warn{notation for $<s,r,o>$. Why we use this Notation to extract graph? What it mean?}\\
\OurMODEL{}
\warn{Why $<s, r , o>$ is core structure?} 
}

\subsection{Graph Extraction.}
Graph Extraction aims to extract the core substructure of the syntactic structure. 
Knowledge graphs provide a highly structured way of representing information by abstracting information into a network of relationships between entities.

Knowledge Graph can be represented as $\mathcal{KG}=\{(s,r,o)\subseteq\mathcal{E}\times\mathcal{R}\times\mathcal{E}\}$, where $\mathcal{E}$ and $\mathcal{R}$ denote the set of entities and relations.

By extracting knowledge graphs from the original prompts, we can discard non-essential grammatical embellishments and auxiliary details, only retain the entities and relationships that express the core semantics. Knowledge graphs can also ensure standardized language expression, reducing redundancy caused by the diversity of expressions.

The process can


\subsection{Further Compression: sub-graph condensation}
\subsubsection{Deductive Coherence Logic and Multidimensional Knowledge Network}
Sub-graph condensation aims to extract the core substructure of the discourse structure. Based on the mode of knowledge generation within the discourse structure, it can be classified into two types: Deductive Coherence Logic and Multidimensional Knowledge Network.

\textbf{Deductive Coherence Logic.} Deductive Coherence Logic underscores the logical sequence and coherence among individual information units within a paragraph. The informational density of a single unit is not high, and each unit is closely dependent on its context. Knowledge is constructed through logical reasoning and structural connections between information units. Chain-of-thought is a typical example of deductive Coherence Logic.

\textbf{Multidimensional Knowledge Network.} Different from deductive Coherence Logic, each information unit in the Multidimensional Knowledge Network contains high-density knowledge. In addition to linear order, the information unit in Multidimensional Knowledge Network can also be connected in a more flexible way to form a more complex knowledge network. Question Answering is a typical example of Multidimensional Knowledge Network.

\subsubsection{Sub-graph condensation}
Each information unit in Deductive Coherence Logic is context-dependent. Any compression may cause the break of the logical chain, so it is not suitable for further compression.\\

Each information unit in the Multidimensional Knowledge Network contains high-density knowledge. Different substructures contain information for different questions, so we can further compress to extract the substructure that is most relevant to the target question.\\



















































